Continual Transformers: Redundancy-Free Attention for Online Inference

Transformers in their common form are inherently limited to operate on whole token sequences rather than on one token at a time. Consequently, their use during online inference on time-series data entails considerable redundancy due to the overlap in successive token sequences. In this work, we propose novel formulations of the Scaled Dot-Product Attention, which enable Transformers to perform efficient online token-by-token inference on a continual input stream. Importantly, our modifications are purely to the order of computations, while the outputs and learned weights are identical to those of the original Transformer Encoder. We validate our Continual Transformer Encoder with experiments on the THUMOS14, TVSeries and GTZAN datasets with remarkable results: Our Continual one- and two-block architectures reduce the floating point operations per prediction by up to 63x and 2.6x, respectively, while retaining predictive performance.

==> contents/8-bios.tex <==

% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author-lukas.jpeg}}]{Lukas Hedegaard}
is a PhD candidate at Aarhus University, Denmark. He received his M.Sc. degree in Computer Engineering in 2019 and B.Eng. degree in Electronics in 2017 at Aarhus University, specialising in signal processing and machine learning. With a common theme of efficient deep learning, his research endeavours span from online inference acceleration and human activity recognition to transfer learning and domain adaptation.
\end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{Name here}
% Biography text here.
% \end{IEEEbiographynophoto}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author-arian-colour-adjusted.jpg}}]{Arian Bakhtiarnia}
Is a PhD student at Aarhus University, Denmark. He received his M.Sc. degree in Algorithms and Computation in 2020 from University of Tehran, Iran and B.Sc. degree in Software Engineering in 2018 from Sharif University of Technology, Iran. His research focuses on computer vision and efficient deep learning.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/author-alexandros.jpg}}]{Alexandros Iosifidis}
(SM'16) is a Professor at Aarhus University, Denmark. He serves as Associate Editor in Chief (for Neural Networks) for Neurocomputing journal, he was an Area Chair for IEEE ICIP 2018-2021 and EUSIPCO 2019,2021, and a Publicity co-Chair of IEEE ICME 2021. He was the recipient of the EURASIP Early Career Award 2021 for contributions to statistical machine learning and artificial neural networks. His research interests focus on neural networks and statistical machine learning finding applications in computer vision, financial modelling and graph analysis problems.
\end{IEEEbiography}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}
